A Comprehensive Empirical Study of Bugs in Open-Source Federated Learning Frameworks

Federated learning (FL) is a distributed machine learning (ML) paradigm, allowing multiple clients to collaboratively train shared machine learning (ML) models without exposing clients' data privacy. It has gained substantial popularity in recent years, especially since the enforcement of data protection laws and regulations in many countries. To foster the application of FL, a variety of FL frameworks have been proposed, allowing non-experts to easily train ML models. As a result, understanding bugs in FL frameworks is critical for facilitating the development of better FL frameworks and potentially encouraging the development of bug detection, localization and repair tools. Thus, we conduct the first empirical study to comprehensively collect, taxonomize, and characterize bugs in FL frameworks. Specifically, we manually collect and classify 1,119 bugs from all the 676 closed issues and 514 merged pull requests in 17 popular and representative open-source FL frameworks on GitHub. We propose a classification of those bugs into 12 bug symptoms, 12 root causes, and 18 fix patterns. We also study their correlations and distributions on 23 functionalities. We identify nine major findings from our study, discuss their implications and future research directions based on our findings.

==> section/2-background.tex <==
\section{Federated Learning Frameworks} \label{sec:background}

% FL paradigm
Federated learning (FL) trains machine learning models across distributed clients (e.g., personal devices or data centers) that are in possession of private data and need to retain it locally. 
Apart from peer-to-peer FL~\cite{RoySPNW19}, most scenarios include a central server who orchestrates the training procedure. 
Typically, the central server distributes a global model initially, then aggregates the updates from clients by an aggregation algorithm and redistributes the aggregated ones again until the convergence or predetermined threshold is reached. 
% Classification of FL
FL can be classified into three categories~\cite{YangLCT19}: horizontal FL, vertical FL and federated transfer learning, by how data is distributed among clients.
Alternatively, it can be divided into two categories~\cite{KairouzMABBBBCC21}: cross-device FL and cross-silo FL, by the types and numbers of clients.
%Figure~\ref{fig:fl-paradigm} demonstrates a common paradigm.

%\begin{figure}[t]
%  \centering
%  \includegraphics[width=0.45\textwidth]{figure/fl-paradigm.pdf}
%  \caption{A simple federated learning paradigm.}
%  \label{fig:fl-paradigm}
%   \Description{}
%\end{figure}

% FL frameworks general architecture and \swj{functional} components
% For the convenience of research and industrial applications, FL frameworks are developed. 
% Different developer teams created distinct FL frameworks according to their ideas and goals. To fulfill their plans and meet the practical requirements, developers and practitioners implemented various \swj{functional} components~\cite{DBLP:journals/csur/LoLWPZ21}.
% Details are given in Table~\ref{tab:\swj{functional}-components-distribution}. 

% FL frameworks general architecture and \swj{functional} components
For the convenience of academic research and industrial applications, various FL frameworks have been released recently. 
Some parts of FL frameworks still adhere to a similar architecture despite of different application scenario targets and according heterogeneous architecture designs.
% In spite of different application scenarios and heterogeneous architecture designs, some parts of FL frameworks still follow a similar architecture. 
%Figure~\ref{fig:fate-arch} shows the architecture of FATE, a representative and popular industrial FL framework.
Based on the similarities and differences of architecture designs of these frameworks, we construct a taxonomy of functionalities, each of which represents a component with a specific function in the FL frameworks. 
% They are divided into two parts: \textbf{core} parts that involve algorithm implementation and functions closely related to FL and \textbf{auxiliary} parts that are designed for extensibility, scalability or user-friendliness etc., of the FL frameworks.
Details are given in Table~\ref{tab:functional-components-distribution}.

% brief intro about these frs

% % A figure for general architecture
% \begin{figure}%[h]
%   \centering
%   \includegraphics[width=\linewidth]{figure/fate_architecture_overview.png}
%   \caption{The architectures of FATE.}
%   \label{fig:fate-arch}
% %   \Description{}
% \end{figure}



==> section/5-discussion.tex <==
\section{Discussion} \label{sec:discussion}
% (Summarize the findings)
% (Advice; Possible solutions)
The findings observed in the study are thoroughly discussed in this section, along with a summary of their implications. Additionally, we propose potential solutions based on the derived implications from our results.

\subsection{For Researchers on Bugs}
% {\bfseries For Researchers on Bugs.}
% The prevailing root cause is \textit{Logic Error}, leading to 421/1,112 (37.9\%) bugs. Such bugs typically involve multiple lines or blocks of code. Consequently, the need arises for automated bug localization and fixing tools capable of effectively addressing issues spanning dozens of lines of code.

% Additionally, developers' misunderstandings contribute to a portion of bugs attributed to \textit{Logic Error}. Inconsistencies between the implemented functions and the expected behavior are their typical manifestations.
% % Furthermore, a considerable portion of bugs caused by \textit{Logic Error} result from the inconsistencies between the implemented functions and the expected ones, which usually stems from developers' misunderstandings. 
% Under such circumstances, a lightweight automated consistency checking tool is beneficial to developer teams following agile software development principles~\cite{beck2001manifesto, WilliamsC03}. This kind of tool should be able to utilize simple specification files to define the expected functions and perform continuous checks throughout the development process.

% The results of the correlation analysis highlight significant independence between the most common symptoms and root causes of bugs.
% This implies that relying solely on the presence of bug symptoms provides limited assistance in accurately identifying potential root causes.
% This poses a challenge for both manual and automatic analyses in pinpointing potential root causes in presence of bug symptoms. 
% In addition, findings from cross analysis of distributions across functionalities and application scenarios indicates the widespread dominance of the most frequent symptoms, root causes and fix patterns. 

Moreover, the distributions across functionalities correspond to the challenge posed by heterogeneous architectures in different FL frameworks. The auxiliary functionalities are proven to be the most bug-prone ones based on the distribution data.
% Additionally, the finding from bug distributions on functionalities correspond to the challenge posed by heterogeneous architectures we encountered that FL framework architectures vary a lot in these customized auxiliary functionalities, which are now proved by the distribution data to be the most bug-prone components. 
% As the auxiliary functionalities of FL frameworks are loosely connected to features of FL, they share similarities in architecture designs to those in other software systems. 
% Consequently, mature approaches that have been successfully applied to those systems are likely to exhibit proficiency in identifying and resolving bugs present in the auxiliary functionalities.

\subsection{For Maintainers of Frameworks}
% \noindent {\bfseries For Maintainers of Frameworks.}
The findings demonstrate a consistent relationship among symptoms, root causes, and fix patterns. 
They jointly reflect the presence of \textit{disorganized pull requests and ambiguous bug descriptions}. 
Specifically, many bugs with unclear accounts of symptoms are attributed to \textit{Functional Error}, the symptom covering the largest number of bugs. This widens the gap in the numbers of bugs between \textit{Function Error} and \textit{Crash}, which is the second most frequent symptom.
% Similarly, concerning root causes, \textit{Logic Error} covers the largest number of bugs. Additionally, it is the only root cause that is positively correlated with \textit{Unknown} symptom. Both of them feature complicated modifications of code logic in source files.

Considering the intrinsic complexity of bugs in the aforementioned categories, the disorganized pull requests, alongside ambiguous descriptions of root causes and symptoms, contribute greatly to the probabilities of false positives in the classification results.
% If the pull requests are more organized, and symptoms and root causes are clearly explained, there is likely to be fewer false positives particularly in \textit{Functional Error}, \textit{Logic Error} and \textit{Unknown}.

Given that all the bugs are collected from the initial release of each FL framework as open-source, the imperfect management of bug reports in these frameworks serve as indications of the intense competition among the frameworks during the early stage of development. As the developers prioritize the delivery of practicable frameworks, they pay less attention to the clarity of the bug reports.
% These observations provide valuable insights into the possible adoption of agile software development approaches by the developers
% They act as clues to the possible agile software development~\cite{beck2001manifesto, WilliamsC03} approaches adopted by the developers. 

We suggest that developers should enforce a more rigorous bug reporting produce and try to clarify pull requests with bug-fixing modifications.

Furthermore, in light of a considerable quantity of bug-related pull requests where incorrect intermediate results in the source files are manifest but the symptoms are vaguely described,
% which are classified into \textit{Functional Error}, 
more assertions checking the intermediate results should be added to the source files to incur crashes as earlier as possible.




==> section/9-acknowledgments.tex <==
\section{Acknowledgments}  \label{sec:Acknowledgments}
To Robert, for the bagels and explaining CMYK and color spaces.
